On Coherence in Bragg-Primakoff Axion Photoconversion

Axions and axion-like pseudoscalar particles with dimension-5 couplings to photons exhibit coherent Bragg-Primakoff scattering with ordered crystals at keV energy scales. This provides for a natural detection technique in searches for axions produce in the Sun's interior. I will motivate the utility of dark matter direct detection experiments in searching for solar axions, emphasizing the role crystal-based detector technologies. I present an updated theoretical treatment of the Bragg-Primakoff photoconversion process for keV pseudoscalars, and address simultaneously the effects of absorption of final state photons in crystals on the loss of coherence, which can lead to large suppressive corrections to the event rate sensitivity for this detection technique. However, I also show that the Borrmann effect of anomalous absorption significantly lifts the suppression. This phenomenon is studied in Ge, NaI, and CsI crystal experiments and its impact on the the projected sensitivities of SuperCDMS, LEGEND, and SABRE to the solar axion parameter space. Lastly, I investigate the future reach of multi-ton scale crystal detectors and discuss strategies to maximize the discovery potential of experimental efforts in this vein.

==> data/nomenclature.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
%  New template code for TAMU Theses and Dissertations starting Fall 2016.  
%
%
%  Author: Sean Zachary Roberson
%  Version 3.17.09
%  Last Updated: 9/21/2017
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%                           NOMENCLATURE
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\chapter*{NOMENCLATURE}
\addcontentsline{toc}{chapter}{NOMENCLATURE}  % Needs to be set to part, so the TOC doesnt add 'CHAPTER ' prefix in the TOC.

%A note about aligning: These entries will align
%themselves according to the ampersand (&).
%No extra spaces are needed, as seen in some of
%the entries below.

%Example of the longtable environment.
\hspace*{-1.25in}
\vspace{12pt}
\begin{spacing}{1.0}
	\begin{longtable}[htbp]{@{}p{0.35\textwidth} p{0.62\textwidth}@{}}
	   % \begin{tabular}{@{}p{0.33\textwidth} p{0.62\textwidth}@{}}
		OGAPS	&	Office of Graduate and Professional Studies at Texas A\&M University\\	[2ex]
		B/CS		&	Bryan and College Station\\	[2ex] %[2ex] provides double space between each row
		TAMU			&	Texas A\&M University\\	[2ex]
		SDCC & San Diego Comic-Con\\ [2ex]
		EVIL & Every Villain is Lemons\\ [2ex]
		EPCC & Educator Preparation and Certification Center at Texas A\&M University - San Antonio\\ [2ex]
		FFT & Fast Fourier Transform\\ [2ex]
		ARIMA & Autoregressive Integrated Moving Average\\ [2ex]
		SSD & Solid State Drive\\ [2ex]
		HDD & Hard Disk Drive\\ [2ex]
		O\&M & Eller Oceanography and Meteorology Building\\ [2ex]
		DOS & Disk Operating System\\ [2ex]
		HDMI & High Definition Multimedia Interface\\ [2ex]
		$L^1$ & Space of absolutely Lebesgue integrable functions; i.e., $\int |f| < \infty$\\ [2ex]
		$L^2$ & Space of square-Lebesgue-integrable functions, i.e., $\int |f|^2 < \infty$\\ [2ex]
		$PC(S)$ & Space of piecewise-continuous functions on $S$\\ [2ex]
		GNU & GNU is Not Unix\\ [2ex]
		GUI & Graphical User Interface\\ [2ex]
		PID & Principal Integral Domain\\ [2ex]
		MIP & Mixed Integer Program\\ [2ex]
		LP & Linear Program\\ [2ex]
		%XXXXXXXX		&	This is an optional page. Random word to test how long the sentence can be? This is just for test purpose. The current setting aims to align left/right margin same as all other pages.\\	[2ex]
	   % \end{tabular}%
	\end{longtable}
\end{spacing}

\pagebreak{}
